An Adaptive Black-box Defense against Trojan Attacks (TrojDef)

Trojan backdoor is a poisoning attack against Neural Network (NN) classifiers in which adversaries try to exploit the (highly desirable) model reuse property to implant Trojans into model parameters for backdoor breaches through a poisoned training process. Most of the proposed defenses against Trojan attacks assume a white-box setup, in which the defender either has access to the inner state of NN or is able to run back-propagation through it. In this work, we propose a more practical black-box defense, dubbed TrojDef, which can only run forward-pass of the NN. TrojDef tries to identify and filter out Trojan inputs (i.e., inputs augmented with the Trojan trigger) by monitoring the changes in the prediction confidence when the input is repeatedly perturbed by random noise. We derive a function based on the prediction outputs which is called the prediction confidence bound to decide whether the input example is Trojan or not. The intuition is that Trojan inputs are more stable as the misclassification only depends on the trigger, while benign inputs will suffer when augmented with noise due to the perturbation of the classification features. Through mathematical analysis, we show that if the attacker is perfect in injecting the backdoor, the Trojan infected model will be trained to learn the appropriate prediction confidence bound, which is used to distinguish Trojan and benign inputs under arbitrary perturbations. However, because the attacker might not be perfect in injecting the backdoor, we introduce a nonlinear transform to the prediction confidence bound to improve the detection accuracy in practical settings. Extensive empirical evaluations show that TrojDef significantly outperforms the-state-of-the-art defenses and is highly stable under different settings, even when the classifier architecture, the training process, or the hyper-parameters change.

==> related.tex <==
\section{Related Work}\label{sec:related}

To defend against the Trojan attack, researchers propose different kinds of methods. To the best of our knowledge, until now, there is no dominant solution that performs consistently better than others. Based on our review, we classify the defense methods against the Trojan attack into the white-box and black-box categories.


\subsection{White-box Defense}

As indicated by the name, this category of defense methods treats the NN classifiers as white-box models. In other words, these methods build their defense on top of the inner information that the NN classifier provided. For example, in \cite{liu2018fine}, the researchers introduce a defense that is called Fine-Pruning. This defense assumes that the NN classifier is infected by the Trojan attack. To eliminate the implanted backdoor, it first removes the redundant connections in the NN classifier. Then, the second step is to fine-tune the modified NN classifier with extra training data. Moreover, in defense methods \cite{chou2018sentinet} and \cite{doan2019februus}, the gradient information from the NN classifier is used to isolate the most influential area.

Although these defense methods are shown to defend the Trojan attack, there are still unsolved issues. Among these issues, these defense methods share a common problem of assuming the NN classifier as a white-box model. In real-world scenarios, the NN classifiers are usually provided as a black-box model, only allowing the defense to run forward-pass, making these methods not practical.

\subsection{Black-box Defense}

As described above, black-box defenses are more practical for real-world applications. To the best of our knowledge, the SOTA black-box defense against the Trojan attack is STRIP introduced in \cite{gao2019strip}. It superimposes each input image with several prepared benign images (i.e., hold-out data) and then generates the corresponding predictions by feeding them to the NN classifier. Recall that the Trojan trigger in the attack example can mislead the NN classifier to classify any input to the target class. As a result, if the input example contains the Trojan trigger, the predictions on different superimposition should be more stable than that of the benign example. Lastly, STRIP utilizes the calculated Entropy and a selected threshold to distinguish Trojan inputs from benign ones.

Although STRIP is a black-box defense against the Trojan attack, it is not an effective approach and contains unresolved issues. For example, STRIP does not clearly describe the connection between the Trojan example and the Entropy calculation. Moreover, from our evaluation, we also noticed that the superimposition process utilized in STRIP is hard to be generalized to different settings (e.g., the NN architectures, the Trojan triggers, and the datasets).
